Structure Editor for Building Software Models

Alloy is well known a declarative modeling language. A key strength of Alloy is its scenario finding toolset, the Analyzer, which allows users to explore all valid scenarios that adhere to the model's constraints up to a user-provided scope. Despite the Analyzer, Alloy is still difficult for novice users to learn and use. A recent empirical study of over 93,000 new user models reveals that users have trouble from the very start: nearly a third of the models novices write fail to compile. We believe that the issue is that Alloy's grammar and type information is passively relayed to the user despite this information outlining a narrow path for how to compose valid formulas. In this paper, we outline a proof-of-concept for a structure editor for Alloy in which user's build their models using block based inputs, rather than free typing, which by design prevents compilation errors.

==> casestudy.tex <==
\section{Illustrative Example}
To illustrate how a structure editor can have a practical impact, we highlight how a structure editor would overcome the limitations from our motivating examples.

\subsection{Preventing Syntax Errors - inv5}


\subsection{Preventing Type Errors - inv10}


%For these edits, once the user adds the \CodeIn{always} operator on line 16, the structure editor will not let the user add ``\CodeIn{Protected once}'', but rather give the user a list of options to build a proper boolean formula, such as ``\CodeIn{Protected in [...]}'' or  These options could make the user think to backtrack by removing ``\CodeIn{Protected}'' and reformulating to ``\CodeIn{some Protected}.''

==> figures/trash.tex <==
\usetikzlibrary{shapes.geometric, arrows}
\tikzstyle{arrow} = [line width=1.5pt,->,>=stealth]
\tikzstyle{darrow} = [line width=1.5pt,<->,>=stealth]
\tikzstyle{ListAtom} = [rectangle, minimum width=1.25cm, minimum height=.7cm, text centered, draw=black, fill=orange!75!yellow]
\tikzstyle{Trash} = [rectangle, minimum width=1.25cm, minimum height=.7cm, text centered, draw=black, fill=white!50!red]
\tikzstyle{Protected} = [rectangle, minimum width=1.25cm, minimum height=.7cm, text centered, draw=black, fill=yellow!75!orange]
\tikzstyle{State} = [circle, minimum width=0.5cm, minimum height=0.5cm, text centered, draw=black, fill=white]

\begin{figure*}
\begin{center})
\begin{tabular}[t]{c|c}
%\footnotesize (a) &  \footnotesize (c) \\

\begin{minipage}[t]{.6\columnwidth}
\scriptsize
\begin{Verbatim}[]
                     \textrm{\footnotesize{(a)}}
\Blue{var sig} File \{ \Blue{var} link : \Blue{lone} File \}
\Blue{var sig} Trash \Blue{in} File \{\}
\Blue{var sig} Protected \Blue{in} File \{\}

__________________________________________________
                     \textrm{\footnotesize{(b)}}

\Green{//links will eventually be in the trash}
\Blue{pred} inv8 \{ \Blue{eventually} link {\setlength{\fboxsep}{1pt}\colorbox{red!30}{\Blue{in}}} Trash \}
\textit{A type error has occured: in can be used only}
\textit{between 2 expressions of the same arity.}
\textit{Left type = {this/File->this/File}}
\textit{Right type = {this/File}}
\end{Verbatim}
\end{minipage}

& 

\begin{minipage}[t]{1.1\columnwidth}
\scriptsize
\begin{Verbatim}[]
                                \textrm{\footnotesize{(c)}}
\Green{//initially the trash is empty and there are no protected file}
\Blue{pred} inv1 \{ \Blue{no} Trash & {\setlength{\fboxsep}{1pt}\colorbox{red!30}{\Blue{no}}} Protected \}
\textit{Syntax error at line [x] column [y]:} 
\textit{There are 28 possible tokens that can appear here: [...]}

\Green{//whenever a file is sent to the trash, it remains in there forever}
\Blue{pred} inv6 \{ \Blue{all} f:Trash | {\setlength{\fboxsep}{1pt}\colorbox{red!30}{\Blue{always}}} f \}
\textit{A type error has occured:}
\textit{This expression failed to be typechecked line [x] column [y]}

\Green{//the protected status never changes}
\Blue{pred} inv10 \{ \Blue{always} {\setlength{\fboxsep}{1pt}\colorbox{red!30}{\Blue{all}}} Protected \}
\textit{Syntax error at line [x] column [y]:} 
\textit{The "all x" construct is no longer supported.}

\Blue{pred} inv10 \{ {\setlength{\fboxsep}{1pt}\colorbox{red!30}{\Blue{once}}} Protected \Blue{always} Protected \}
\textit{A type error has occured:}
\textit{This expression failed to be typechecked line [x] column [y]}
\end{Verbatim}
\end{minipage}


\end{tabular}


\end{center}
\caption{Faulty Submission of an Alloy Model of a File System Trash Can}
\label{fig:trash}
\end{figure*}
